DETOX: A Redundancy-based Framework for Faster and More Robust Gradient Aggregation

To improve the resilience of distributed training to worst-case, or Byzantine node failures, several recent approaches have replaced gradient averaging with robust aggregation methods. Such techniques can have high computational costs, often quadratic in the number of compute nodes, and only have limited robustness guarantees. Other methods have instead used redundancy to guarantee robustness, but can only tolerate limited number of Byzantine failures. In this work, we present DETOX, a Byzantine-resilient distributed training framework that combines algorithmic redundancy with robust aggregation. DETOX operates in two steps, a filtering step that uses limited redundancy to significantly reduce the effect of Byzantine nodes, and a hierarchical aggregation step that can be used in tandem with any state-of-the-art robust aggregation method. We show theoretically that this leads to a substantial increase in robustness, and has a per iteration runtime that can be nearly linear in the number of compute nodes. We provide extensive experiments over real distributed setups across a variety of large-scale machine learning tasks, showing that DETOX leads to orders of magnitude accuracy and speedup improvements over many state-of-the-art Byzantine-resilient approaches.

==> ConvergenceRates.tex <==
%!TEX root = DETOX_neurips.tex
\section{Convergence Rates}\label{section:convergence_new}
In \cite{yin2018byzantine,DBLP:journals/corr/abs-1806-05358}, the authors provide convergence rates for Byzantine tolerant gradient descent for Trimmed Mean and Iterative Filtering estimators. \cite{DBLP:journals/corr/abs-1806-05358} defines $\Delta$-inexact gradient oracle as:
\begin{definition}
 An estimator $Aggr$ provides a $\Delta$-inexact gradient oracle for the true population loss gradient $g$ if $\|Aggr - g\|\leq \Delta$.
\end{definition}
Note that in the setting of \cite{yin2018byzantine,DBLP:journals/corr/abs-1806-05358}, the papers consider that each worker machine computes gradients on $p$ data points are returns the mean gradient. In our setting, a Block of size $r$ computes $r$ gradients, that is 1 data point on average per machine. We can easily extend this to their setting (each block of size $r$ will compute gradients on $pr$ points) and we will see correspondingly more accurate gradients. However, for the sake of exposition, we assume that each machine computes $r$ gradients and not $pr$ gradients.
\paragraph*{Trimmed Mean} \cite{yin2018byzantine} gives the following result:
\begin{theorem} \cite{yin2018byzantine}
Trimmed Mean is a $\Delta$-inexact gradient oracle, with $\Delta = \mathcal{O}\left( d \left(x +\dfrac{1}{n}\right) \right)= \mathcal{O}\left( d x \right)$ where we ignore the logarithmic terms. 
\end{theorem}
Using Corollary \ref{lemma:5}, we see that after using \dracolite{} $x_e \to 0$ and thus, the effective $\Delta_e$
\begin{cor} 
For Trimmed Mean, after using \dracolite{}: $\Delta_e = \mathcal{O}\left( \dfrac{d}{n}\right)$. Again, we ignore the logarithmic terms. 
\end{cor}

\paragraph*{Iterative Filtering} \cite{DBLP:journals/corr/abs-1806-05358} gives the following result for iterative filtering \cite{diakonikolas2017being}:
\begin{theorem} \cite{DBLP:journals/corr/abs-1806-05358}
For Iterative Filtering, $\Delta = \mathcal{O}\left(  \left(\sqrt{x} +\sqrt{\dfrac{d}{n}}\right) \right)$ where we ignore the logarithmic terms. 
\end{theorem}
Again, using Corollary \ref{lemma:5}, we see that after using \dracolite{} $x_e \to 0$ and thus, the effective $\Delta_e$
\begin{cor} 
For Iterative Filteringn, after using \dracolite{}: $\Delta_e = \mathcal{O}\left( \sqrt{\dfrac{d}{n}}\right)$. Again, we ignore the logarithmic terms. 
\end{cor}

% \section{(Old, needs to be changed) Error Rates}\label{section:convergence}
%   In \cite{yin2018byzantine}, two aggregators are considered: coordinate wise median and coordinate wise trimmed mean. The rate for coordinate wise median provided is independent of the fraction of byzantine machines if the dimension is much higher than the number of machines. Thus, we focus on coordinate wise trimmed mean. Theorem 4 from that paper gives the statistical error rate of trimmed mean under strongly convex loss as $\tilde{\mathcal{O}}\left(\frac{cxd}{\sqrt{p}} + \frac{d}{\sqrt{np}}\right)$ where $c$ is a user chosen constant, $x$ is ratio of Byzantine machines, $d$ is the dimension, $n$ is the number of machines, and $p$ is the number of data points per machine. Theorems 5 and 6 give similar rates under different settings. To adapt \dracolite{} to their setting, note that the difference is that now, each machine computes gradients of $r$ data points. To handle this, we can modify \dracolite{} so that instead of computing $r$ gradients in each block, we compute $pr$ gradients. Now, we can view the output of \dracolite{} as equivalent to a setting where each block is viewed as a single machine: number of machines is now $n/r$, number of data points per machine is $pr$ and $x$ changes to $\gamma_r x$. In this setting the error rate becomes $\tilde{\mathcal{O}}\left(\frac{cd \gamma_r x}{\sqrt{pr}} + \frac{d}{\sqrt{np}}\right)$. Now, using Lemma \ref{lemma:2} it can be seen that this becomes $\tilde{\mathcal{O}}\left(\frac{c'd (x(1-x))^{(r-1)/2} x}{\sqrt{pr}} + \frac{d}{\sqrt{np}}\right)$ which can be driven arbitrarily close to $\tilde{\mathcal{O}}\left(\frac{d}{\sqrt{np}}\right)$ by increasing $r$. We see that $r\approx \tilde{\mathcal{O}}(-\log(n)/\log(x(1-x)))$ for this.\\
% Another interesting analysis from \cite{yin2018byzantine} is when the Robust One-round algorithm is run on a convex quadratic function. Each machine minimizes the loss function and sends its final parameters to the parameter server which takes the coordinate wise median (See Algorithm 2 in the paper for details). This involves just one round of communication between the parameter servers and the worker machines. Theorem 7 from the paper says that the error in the learnt model: $\|\hat{w}-w^*\|$ is $\mathcal{O}({\frac{x}{\sqrt{p}} + \sqrt{\frac{\log(npd)}{2n(1-x)}} + \frac{\tilde{C}}{\sqrt{p}}})$ where $\tilde{C}$ is a constant. Now, consider only the dominant term :$\mathcal{O}(\frac{x}{\sqrt{p}})$. This can be reduced by using \dracolite{} to $\mathcal{O}\left(\frac{x(x(1-x))^{(r-1)/2}}{\sqrt{pr}}\right)$.

==> ImprovingRobustness.tex <==
%!TEX root = draco_lite_neurips.tex
\section{(Old, needs to be removed?)Improving robustness guarantees and speeding up aggregators}\label{section:speedup}
For this section, we assume that the number of byzantine machines has been reduceds to a small constant $c$ as compared to the total number of machines. Please see section \ref{section:constq} where we describe our technique to achieve this.\\
We know that finding mean is a really fast aggregation (and it has distributed implementations as well). But unfortunately it is not robust to byzantine attacks. We show that any aggregator can be used to achieve the time complexity of mean, while improving robustness guarantees.\\
% \subsection{Error rate improvements}
Let us run any aggregator on random sets of gradients (let's call them buckets) of size $4c + k$ (Instead of '$4$', we can take any arbitrary constant greater than 2. We took 4 to ease our calculations). Now, each of these buckets can be expected to return a robust aggregate of the gradients.\\
 Given this setup, the number of byzantine machines in each group can vary from $0$ to $c$. Therefore, $x$ varies from $0$ to $0.25$.\\
 % Given this, from Section \ref{section:convergence}, we can see that the error rate of each bucket becomes $\tilde{\mathcal{O}}\left(\frac{d}{\sqrt{pr}}\right)$. If originally $x$ was $\mathcal{O}(1)$, this is of the same order as trimmed mean applied directly (which is $\tilde{\mathcal{O}}\left(\frac{xd}{\sqrt{p}}\right)$). If we take the mean across the bucket, the error rate still remains $\tilde{\mathcal{O}}\left(\frac{d}{\sqrt{pr}}\right)$.

\subsection{Inner product methods}
\begin{definition}
\textbf{$(\alpha,q)$-Byzantine Resilience\cite{blanchard17} :} Let $0 \leq \alpha < \pi/2$ be any angular value, and any integer $0 \leq q \leq n$. Let $\{v_i: i \in [n]\}$ be any i.i.d. random vectors in $R^d$, $v_i \sim G$, with $\E[G] = g$. Let $\{\tilde{v}_i: i \in [n]\}$ be the set of vectors, of which up to $q$ of them are replaced by arbitrary vectors in $R^d$, while the others still equal to the corresponding $\{v_i\}$. Aggregation rule $Aggr(\cdot)$ is said to be classic $(\alpha, q)$-Byzantine resilient if 
$
Aggr(\{\tilde{v}_i: i \in [n]\})
$
satisfies (i) $\langle{\E[Aggr]},{g}\rangle \geq (1-\sin \alpha) \|g\|^2 > 0$ and (ii) for $r = 2,3,4$, $\E\|Aggr\|^r$ is bounded above by a linear combination of terms $\E\|G\|^{r_1}, \ldots, \E\|G\|^{r_{n-q}}$ with $r_1 + \ldots + r_{n-q} = r$.
\end{definition}
We know that most robust aggregators (see examples below) are $(\alpha, q)$ - Byzantine resilient when $n\geq2q+k$ (where $k$ is some constant depending on the aggregator).\\

\begin{algorithm}
	\caption{Improve speed and robustness of aggregator}
    \begin{algorithmic}[1]
    \INPUT $n$ machines and $n$ data points; aggregator $A$ with robustness requirement $n \leq 2q + k$
    % \STATE \textbf{Ensure: } $q/n<0.5$
    \REPEAT{}
        \STATE Use Algorithm 1 to reduce effective number of byzantine machines to constant, that is $q_e = c$
        \STATE Partition the $n$ gradients into 'buckets' of size $4c+k$.
        \STATE Run the aggregator $A$ on the $4c+k$ gradients in each bucket. Let us denote $A_i$ to be the aggregated gradient from bucket $i$.
        \STATE Collect all the $A_i$'s and take their mean.
        \STATE Use the mean to take a step of gradient descent.
    \UNTIL{Convergence}
  \end{algorithmic}
\end{algorithm}

\subsection{Improving robustness guarantees}
As proved in \cite{xie18}, geometric median, marginal median and mean-around-median have $sin(\alpha) \leq \sqrt[]{n}f(x)\left(\dfrac{\sqrt[]{d}\sigma}{\|g\|}\right)$ where:
\begin{enumerate}
\item $f(x) = \dfrac{\sqrt[]{2}(1-x)^{1.5}}{1-2x}$ for geometric median
\item $f(x) = \sqrt[]{1-x}$ for marginal median
\item $f(x) = \sqrt[]{10(1-x)}$ for mean-around-median
\end{enumerate}
Note that $1 \leq f(x) \leq \sqrt[]{7.5} $ for $0 \leq x \leq 0.25 $ for these aggregators.\\
For Krum\cite{blanchard17}, $$sin(\alpha) \leq \sqrt[]{2n +2(nx)^2\dfrac{1-x}{1-2x-\frac{2}{n}}}\left(\dfrac{\sqrt[]{d}\sigma}{\|g\|}\right)$$\\

Thus, for the aggregators, the bound on $sin(\alpha)$ increases with $n$. This is really bad if n is big. In essence, we are losing guarantee on robustness. On the other hand, as shown above, the range of $x$ is bounded, and thus the dependence on $x$ is bounded and hence it does not affect the bound on $sin(\alpha)$ much.\\
If we form buckets, as described above, $x \leq 0.25$ for each of the buckets, and for bucket $i$, $n_i = 4c + k$. Therefore the '$n$' factor reduces to '$4c + k = O(1)$' whereas the change due to change in $x$ is bounded. Therefore, for each bucket, the robustness guarantee improves.\\
Let's assume depending on $c$ and the aggregator used, we get an upper bound $\alpha$ for each bucket. Since the size of each bucket is same and we have less than $c$ byzantine machines in each bucket, the bound for $\alpha$ for each bucket is the same. Let's say the bound is $\alpha_B$, and the aggregated gradient returned by bucket $i$ is $A_i$. Therefore, the bound on the mean:
\begin{align*}
	\left\langle{\E\left[\dfrac{\sum_{i=1}^{n/(4c+k)}A_i}{n/(4c+k)}\right]},g\right\rangle &= \dfrac{\sum_{i=1}^{n/(4c+k)} \langle{\E[A_i]},g\rangle}{n/(4c+k)}\\	
    % &=  \langle{\E[A_i]},g\rangle\\
     &\geq (1-\sin \alpha_B) \|g\|^2\\	
\end{align*}

\subsection{Speeding up slower aggregators}
We focus on two slow aggregators, but the technique can be extended to any aggregator in general.
The time complexity of Krum (and also multi krum\cite{xie18}) is $O(n^2d)$ and that of Bulyan(A)\cite{mhamdi18} is $O(nC)$ where C is the time complexity of the aggregator $A$.
 Let $C=O(n^m d)$, where $m \geq 0$. Now, these complexities are not desirable if n is big. Our proposed technique can speed this up if the conditions mentioned in section \ref{section:speedup} hold.\\

For Krum, we see that the time complexity for each group would be $O((4c^2+k)^2d)$. Aggregated computational time of the groups would be $\dfrac{n}{4c^2+k}O((4c^2+k)^2d) = O((4c^2+k)nd)$. This gives us $\dfrac{n}{4c^2+k}$ gradients. Once we have the set of these krum gradients, we can use a faster aggregator like mean (which has time complexity $O(n_0d)$ for $n_0$ gradients) on this set and get the final aggregated gradient with the final time complexity $O\left((4c^2+k)nd + \dfrac{nd}{4c^2+k}\right) = O(nd)$ which is the same as mean.\\

The same process can be done for Bulyan(A) (or any other aggregator with time complexity $O(n^md), m\geq 0$) but the bucket size would depend on robustness requirements for Bulyan(A). This would lead to a final time complexity of $O(nd)$, similar to previous case.

We can easily see that any other aggregator can be used here and the final time complexity would still be the same as that of mean. Thus, we have seen that not only does this technique improve speed, it also improves guarantees on robustness.
